Unleash the Potential of Long Semantic IDs for Generative Recommendation

Semantic ID-based generative recommenders face a granularity-efficiency dilemma between efficient recommendation with short IDs and expressive item modeling with long IDs. To break this dilemma, we propose ACERec, a framework that preserves the semantic richness of long IDs while keeping the recommendation process efficient. Concretely, ACERec employs an Attentive Token Merger to compress long semantic IDs into compact yet faithful latent tokens. To better capture user intent from the compressed semantics, we further introduce a dedicated Intent Token, optimized by a dual-granularity objective that combines token-level generation with item-level intent-semantic alignment. Extensive experiments on nine real-world benchmarks show that ACERec consistently outperforms state-of-the-art methods, yielding average relative improvements of 12.92% in NDCG@10 and 7.49% in Recall@10 over the strongest baselines.

==> limitations.tex <==
\section*{Limitations}

Despite the promising results achieved by \modelname{} for efficient and expressive generative recommendation, there are three primary limitations to this study. \textbf{First}, our framework adopts a two-stage pipeline where the discrete item tokenization is pre-computed via OPQ and remains fixed during the sequential training phase. Although our ATM effectively executes soft compression in the continuous latent space, a fully end-to-end joint optimization that dynamically updates discrete tokenization alongside sequential recommenders remains an open challenge. \textbf{Second}, \modelname{} allocates a uniform number of compressed latent tokens (e.g., $k=4$) across all items in the catalog. Consequently, it cannot automatically scale latent capacity according to individual item semantic complexity, potentially introducing minor representation redundancy for structurally simpler items or slight information bottlenecks for exceptionally intricate ones. \textbf{Third}, \modelname{} currently operates on discrete semantic IDs quantized from textual attributes, lacking the capability to utilize multi-modal side information such as text-image pairs. Consequently, extending this attentive merging mechanics to dynamically aggregate cross-modal visual and textual attribute signals remains an unexplored dimension. Overall, while our results are promising, exploring dynamic latent token allocation and scaling \modelname{} to multi-modal scenarios are important next steps toward broader industrial deployment.

\section*{Ethics Statement}

\modelname{} aims to advance efficient and equitable generative recommendation by decoupling tokenization resolution from sequential computational footprints, significantly lowering the algorithmic latency and carbon footprint of deploying high-capacity recommenders over massive item catalogs. We explicitly address the pervasive popularity bias inherent in user behavior distributions through a debiased alignment mechanism, which mitigates the risk of creating rigid feedback filter bubbles and encourages fairer exposure for long-tail items. All evaluations are conducted on publicly available, fully anonymized benchmark datasets and do not involve tracking, collecting, or releasing private or sensitive user data. More broadly, we hope this study motivates future research toward green, resource-efficient recommendation architectures that successfully reconcile representational richness with practical deployment efficiency.
